Implicit Bias and Fast Convergence Rates for Self-attention

We study the fundamental optimization principles of self-attention, the defining mechanism of transformers, by analyzing the implicit bias of gradient-based optimizers in training a self-attention layer with a linear decoder in binary classification. Building on prior studies in linear logistic regression, recent findings demonstrate that the key-query matrix $W_t$ from gradient-descent (GD) converges in direction towards $W_{mm}$, which maximizes the margin between optimal and non-optimal tokens across sequences. However, this convergence is local, dependent on initial conditions, only holds asymptotically as the number of iterations increases, and leaves questions about the potential benefits of adaptive step-size rules unaddressed. To bridge this gap, we first establish scenarios for which convergence is provably \emph{global}. We then analyze two adaptive step-size strategies: normalized GD and Polyak step-size, demonstrating \emph{finite-time} convergence rates for $W_t$ to $W_{mm}$, and quantifying the sparsification rate of the attention map. These findings not only show that these strategies can accelerate parameter convergence over standard GD in a non-convex setting but also deepen the understanding of the implicit bias in self-attention, linking it more closely to the phenomena observed in linear logistic regression despite its intricate non-convex nature.

==> sections/wmm-convergence.tex <==
%\subsection{Directional Convergence}
%\textit{In this section, we consider the case where $\ub$ is fixed, and obtain the rate of convergence of $\frac{\W_t}{\norm{\W_t}}$ to $\frac{\Wm}{\norm{\Wm}}$. Some results also hold when jointly optimizing $\ub$ and $\W$, but rest need to be extended.}



%\subsection{When Assumption \ref{ass:data-score} (two-score condition) holds}
\input{two-score}
%\newpage
% \subsection{When Assumption \ref{ass:data-support} (all tokens are support condition) holds}
% \input{all-support}

